On the Mixed Even-Spin Sherrington-Kirkpatrick Model with Ferromagnetic Interaction

We study a spin system with both mixed even-spin Sherrington-Kirkpatrick (SK) couplings and Curie-Weiss (CW) interaction. Our main results are: (i) The thermodynamic limit of the free energy is given by a variational formula involving the free energy of the SK model with a change in the external field. (ii) In the presence of a centered Gaussian external field, the positivity of the overlap and the extended Ghirlanda-Guerra identities hold on a dense subset of the temperature parameters. (iii) We establish a general inequality between the magnetization and overlap. (iv) We construct a temperature region in which the magnetization can be quantitatively controlled and deduce different senses of convergence for the magnetization depending on whether the external field is present or not. Our approach is based on techniques from the study of the CW and SK models and results in convex analysis.

==> invlat.tex <==


%These are definitions for the preamble of TEX files

%\loadmsbm
%that may be needed for \Bbb (``blackboard bold, Bourbaki'') characters
%\UseAMSsymbols
%
%
%\magnification = \magstep1
\font\tencmmib=cmmib10 \skewchar\tencmmib '60
\newfam\cmmibfam
\textfont\cmmibfam=\tencmmib
\def\Ph{\mathchar'4010}
\def\Ps{\mathchar'4011}
\font\tensmc=cmcsc10
\def\smc{\tensmc}
\def\srm{\sevenrm }
%\font\teneufm=EUFM10
%\font\eighteufm=EUFM10 scaled 800
%\def\Fff#1{\hbox{\teneufm#1}}
%\def\Ffff#1{\hbox{\eighteufm#1}}
\font\tenmsb=msbm10
\font\eightmsb=msbm10 scaled 800
\def\Bbb#1{\hbox{\tenmsb#1}}
\def\Bbbb#1{\hbox{\eightmsb#1}}
%\font\bb=msbm10
%\def{\hbox{\bb N}}
%\def\RR{\hbox{\bb R}}
%\def \NN {{I\kern-.3em N}}
%\def \RR {{I\kern-.3em R}}
\def\bbox{\quad\hbox{\vrule \vbox{\hrule \vskip2pt \hbox{\hskip2pt
\vbox{\hsize=1pt}\hskip2pt} \vskip2pt\hrule}\vrule}}
\def\lessim{\ \lower4pt\hbox{$
\buildrel{\displaystyle <}\over\sim$}\ }
\def\gessim{\ \lower4pt\hbox{$\buildrel{\displaystyle >}
\over\sim$}\ }
\def\n{\noindent}
%\def\P{{\rm P}}
%\def\E{{\rm E}}
%\def\LL{{\cal L}}
\def\n{\noindent}
%\parskip=0.03truein
%\hfuzz=0.2truein
%
%\scriptfont4 = \sevensy
%\scriptscriptfont4 = \fivesy
%\font \gross=cmbx10 scaled \magstep2
%\font \mittel=cmbx10 scaled \magstep0  
%\font \outline=ocrb10f scaled \magstep1 
%\pageno = 1
\def\AA{{\cal A} }
\def\AAA{{\bf A} }
\def\Aap{(A,\AA ,P)}
\def\alf{\alpha}
\def\anorm{\|^.\|}
\def\AP{\it Ann. Probab. \bf}
\def\bbe{\vskip .15pc\hangindent=.5pc\hangafter=1}
\def\BB{{\cal B} }
\def\bxt{\boxtimes}
\def\CC{{\cal C} }
\def\claw{\Rightarrow}
\def\cntr{\centerline}
\def\cosph{\cos\phi}
\def\costh{\cos\theta}
\def\DAN{Dokladi AN Ukr.SSR}
\def\DD{{\cal D} }
\def\dc{{\buildrel {d}\over \longrightarrow}}
\def\defn{\skb\fl Definition\rm. }
\def\dens{\text{dens}}
\def\densC{\dens(\CC)}
\def\Dl{\Delta}
\def\dl{\delta}
\def\dnar{\downarrow}
\def\dpo{d_{P,1}}
\def\dpno{d_{P_n,1}}
\def\dpt{d_{P,2}}
\def\EE{{\Bbb E} }
\def\eee{\ =\ }
\def\eeq{\ \equiv \ }
\def\endp{\vfill\break}
\def\Eng{English transl.:}
\def\eps{\varepsilon}
\def\FF{{\cal F} }
\def\GG{{\cal G} }
\def\gee{\ \ge \ }
\def\goin{\to \infty}
\def\go0{\to 0}
\def\grad{\triangledown}
\def\fl{\smallskip}
%\def\fl{\flushpar} 
\def\HH{{\cal H} }
\def\inv{^{-1}}
\def\JJ{{\cal J} }
\def\KK{{\cal K} }
\def\la{\langle}
\def\li{< \infty}
\def\linF{\ell\upin(\FF)\ }
\def\lm{\lambda}
\def\Lm{\Lambda}
\def\lee{\ \le \ }
\def\leftitem#1{\item{\hbox to\parindent{\enspace#1\hfill}}}
\def\LL{{\cal L} }
\def\Lt{L^2(P)}
\def\Lto{L^2_0(P)}
\def\mc{m^{\CC }(}
\def\mcn{m^{\CC}(n)}
\def\mdsk{\medskip}
\def\mm{\vskip 1mm}
\def\MM{{\cal M} }
\def\nF{\|_{\FF}}
\def\NN{{\cal N} }
\def\normf{\|\cdot\|_{\cal F}}
\def\omg{\omega}
\def\Omg{\Omega}
\def\Omgap{(\Omg,\AA,{\rm Pr})\ }
\def\Omgsp{(\Omg, \Sigma ,{\rm Pr})\ }
\def\Omgspb{(\hat \Omg, \hat \Sigma ,\hat Pr)\ }
\def\Omgspr{(\Omg_{\eps }, \Sigma_{\eps } ,Pr_{\eps })\ }
\def\Omgspp{(\Omg_{\nu }, \Sigma_{\nu } , Pr_{\nu })\ }
\def\OO{{\bf O}}
\def\pard{\partial}
\def\pf{\hfill\break\bf Proof. \rm}
\def\pl{\ + \ }
\def\PP{{\cal P} }
\def\pr{probability}
\def\prm{^{\prime}}
\def\prc{{\buildrel {p}\over \longrightarrow}}
\def\prloc{{\buildrel {p,loc}\over \longrightarrow}}  
\def\prbloc{{\buildrel {{p, bloc}}\over \longrightarrow}}  
\def\qed{\hfill\break\rightline{$\bbox$}}
\def\QQ{{\cal Q}}
\def\ra{\rangle} 
\def\rbar{\overline{\Bbb R}}
\def\refs{\mdsk\cntr {REFERENCES}\mdsk}
\def\RR{{\Bbb R }}
\def\rtar{\Rightarrow}
\def\Ru{(in Russian)\ }
\def\sap{(S,\AA ,P)}
\def\soc{S(\CC )}
\def\setm{\setminus}
\def\sg{\sigma}
\def\sga{$\sigma$-algebra }
\def\sgal{$\sigma$-algebra}
\def\sg2{\sigma^2}
\def\sinph{\sin\phi}
\def\sinth{\sin\theta}
\def\skb{\medskip\fl\bf}
\def\sqt{^{1/2}}
\def\Sp{{\cal SP}(\RR^d)}
\def\SS{{\cal S} }
\def\SSSi{\smallint^{\infty}}
\def\SSOI{\smallint^1_0}
\def\SSS{\smallint}
\def\SSSW{\smallint^{\infty}_{-\infty}}
\def\tens{\otimes}
\def\TVMS{Teoria verojatnostej i matemati\v ceskaia statistika }
\def\TPA{\it Theor. Probability Appl. \bf}
\def\TPMS{Probability Theory and Mathematical Statistics, American
Mathematical Society} 
\def\tpr{\text{Pr}}
\def\TT{{\cal T} }
\def\subin{\_{\infty}}
\def\sumi{\sum^{\infty}}
\def\UMZ{Ukrainskij matemati\v ceskij \v zurnal}
\def\upar{\uparrow}
\def\upin{^{\infty}}
\def\VV{{\cal V}} 
\def\vc{Vapnik-\v Cervonenkis\ }
\def\wc{{\buildrel {w}\over \longrightarrow}}
\def\wloc{{\buildrel {w,loc}\over \longrightarrow}}  
\def\wbloc{{\buildrel {w, bloc }\over \longrightarrow}} 
\def\WW{{\cal W} } 
\def\XX{{\bf X} }
\def\xa{(\XX,\AA )\ }
\def\xap{(\XX,\AA,P)\ }
\def\xy{\{x,y\}}
\def\ZW{\it Z. Wahrscheinlichkeitsth. verw. Geb. \bf}
\def\ZZ{{\cal Z} }
\def\__{_{\infty}}
%\medskipamount=6pt plus 2pt minus 2pt










